Rate-compatible LDPC Codes based on Primitive Polynomials and Golomb Rulers

We introduce and study a family of rate-compatible Low-Density Parity-Check (LDPC) codes characterized by very simple encoders. The design of these codes starts from simplex codes, which are defined by parity-check matrices having a straightforward form stemming from the coefficients of a primitive polynomial. For this reason, we call the new codes Primitive Rate-Compatible LDPC (PRC-LDPC) codes. By applying puncturing to these codes, we obtain a bit-level granularity of their code rates. We show that, in order to achieve good LDPC codes, the underlying polynomials, besides being primitive, must meet some more stringent conditions with respect to those of classical punctured simplex codes. We leverage non-modular Golomb rulers to take the new requirements into account. We characterize the minimum distance properties of PRC-LDPC codes, and study and discuss their encoding and decoding complexity. Finally, we assess their error rate performance under iterative decoding.

==> Figures/figura_matrice.tex <==
\resizebox{0.9\columnwidth}{!}{

\begin{tikzpicture}
  \node (rect1) [rectangle, minimum height=1cm, minimum width=2cm] {
    \begin{tikzpicture}
      
      \fill[gray!80] (0,1.5) -- (1.5,1.5) -- (3,0) -- (1.5,0) -- cycle; % diagonal band
      \draw (0,0) rectangle (3,1.5); % draw rectangle
      \node[below,scale=0.9] at (1.5,-0.1) {$R=1/2$}; % equation
    \end{tikzpicture}
  };
  \node (rect2) [ rectangle, minimum height=1cm, minimum width=2cm, right=of rect1] {
    \begin{tikzpicture}
      
      \fill[gray!80] (0,2) -- (1.5,2) -- (3.5,0) -- (2,0) -- cycle; % diagonal band
      \draw (0,0) rectangle (3.5,2); % draw rectangle
      \node[below,scale=0.9] at (1.75,-0.1) {$R<1/2$}; % equation
    \end{tikzpicture}
  };
  \node (rect3) [ rectangle, minimum height=1cm, minimum width=2cm, right=of rect2] {
    \begin{tikzpicture}
      \fill[gray!80] (0,1) -- (1.5,1) -- (2.5,0) -- (1,0) -- cycle; % diagonal band
       \draw (0,0) rectangle (2.5,1); % draw rectangle
      \node[below,scale=0.9] at (1.25,-0.1) {$R>1/2$}; % equation
    \end{tikzpicture}
  };
\end{tikzpicture}

}

\begin{comment}
  \draw (0,0) rectangle (2,1); % draw rectangle
  \fill[gray!80] (0,1) -- (1,1) -- (2,0) -- (1,0) -- cycle; % diagonal band

\node[below,scale=0.5] at (1,-0.1) {$R=1/2$}; % equation

\end{comment}

==> convo.tex <==
In this section we provide some preliminary insights on the possibility to obtain convolutional codes from the proposed punctured simplex codes. Constant-length puncturing, as in Fig. \ref{fig:Hpunt} on the right, leads to a convolutional code with asymptotic code rate $R=\frac{1}{2}$ (the asymptotic code rate is reached for a frame length tending to infinity). For a code of this type, owing to self-duality, a code frame of weight $w_h$ always exists. Then, we have the bound $d\leq w_h$. In this case, the blocklength (defined as in \cite{Battaglioni2021}) of the convolutional code is $n_0=2$, the number of information symbols per period is $k_0=1$ and the number of control symbols per period is $r_0=1$. Different asymptotic code rates $R=\frac{k_0}{n_0}$ can be obtained by augmenting or diminishing $k_0$ and $r_0$. More specifically, the elimination of rows in $\6H$ follows the following principle: in any period of length $n_0$, $r_0$ rows are eliminated and $k_0$ rows remain. We can distinguish the case of high rate codes, occurring when $r_0=1$, from the case of low rate codes, occurring when $k_0=1$.

In Fig. \ref{fig:Hconvi}, a pair of transposed syndrome former submatrices are shown for codes with $k=14$ and $R=\frac{1}{2}$, $R=\frac{1}{3}$ and $R=\frac{2}{3}$, respectively. The original simplex code has $\6e=[0,4,11,13,14]$. Each transposed syndrome former submatrix has $n_0$ columns and shifts vertically by $r_0$ rows at each period. Below the submatrices, the first few lowest-weight normalized coefficients $B(w)$ are reported. It is remarkable that these codes are characterized by very small normalized coefficients, and this makes them very promising \cite{Battaglioni2021}. We also notice that at rate $\frac{2}{3}$ the convolutional code exhibits $d=3$, whereas the block code only reaches $d=2$.

\begin{figure}[tb]
    \centering
    \includegraphics[keepaspectratio, width=8.9cm]{Figures/conv.png}
    \caption{Transposed syndrome former matrices of some convolutional codes.}
    \label{fig:Hconvi}
\end{figure}

%As for the possibility of an easy soft-decision decoding also for the convolutional version of the codes we propose, it is guaranteed by the relatively small values of the average column weights and $k$. 

==> numere.tex <==
%\textcolor{cyan}{probabilmente va accorpata a quella sopra in qualche modo, per ora la lascio qui perché segue una filosofia un po' diversa, che non è tanto legata a $\6m$ ma a caratteristiche strutturali}


In this section we show some numerical results. In particular, we choose a parity-check polynomial where $k$ is relatively small (for explanatory purposes) and compute the weight distribution of the \ac{PRC-LDPC} code, validating the theoretical analysis carried out in Section \ref{sec:rules}.

Let us start from the family of \ac{PRC-LDPC} codes obtainable from the parity-check polynomial
\[
h(x)=1+x+x^5+x^{11}+x^{13},
\]
from which the reciprocal
\[
h^*(x)=1+x^2+x^8+x^{12}+x^{13},
\]
can be readily obtained. We have that $\6e=[0,1,5,11,13]$ is a Golomb ruler and the following vector containing separations 
$\6s=[1,4,6,2]$. We thus notice that the conditions in Remarks \ref{rem:rul_ext_other}, \ref{rem:rul_sum} and \ref{rem:rul_int} are satisfied.

By performing polynomial division between $x^N+1$ and $h^*(x)$ we obtain the following portion of $\6m$
\[
\ldots |1111|00000000|\mathbf{10100000100011}|00|1010101| \ldots,
\]
where we distinguish $\6h^*$, marked in bold, surrounded by two all-zero portions of size $2(1+4+6)-13-1=8$ and $2(6+2)-13-1=2$, and two comb-like zones, where symbols one are distant $s_0=1$ positions on the left and $s_{w_h-2}=2$ positions on the right. This corroborates the analysis in Section \ref{sec:rules} and, in particular, in Fig. \ref{fig:zonapettini}. The shown sub-sequence already tells us that  $n(6)>24$, but it is possible to study the distance profile even more in detail.

In fact, in this case we have $r(2)=6$ and therefore $n(2)=19$. By exhaustive search we find $A(2)=3$, and these three codewords belong to Families 1 ($2$ out of $3$) and 2 (the remaining $1$). They are marked in bold in the following portion of $\6m$

\begin{align*}
\ldots10001|\textbf{1000000000010000000}|101001\ldots\\
\ldots100011|\textbf{0000000000100000001}|01001\ldots\\
\ldots1000110|\textbf{0000000001000000010}|1001\ldots\\
\end{align*}

By increasing $n$ to $20$, we get $A(2)=1$, still belonging to Family 2 
\begin{align*}
\ldots100011|\textbf{00000000001000000010}|1001\ldots\\
\end{align*}
According to Corollary \ref{cor:corsidon}, we have $n=21=n(3)$ and indeed $d=3$ and $A(d)=8$, where the following codewords are derived from Families 1 and 2 as described in Lemma \ref{lem:puntu} (applied for increasing, rather than decreasing, values of $n$), % since they appear consecutively in $\6m$
\begin{align*}
\ldots10001|\textbf{100000000001000000010}|1001\ldots\\
\ldots100011|\textbf{000000000010000000101}|001\ldots\\
\end{align*}
and the others belong to new families. Finally, when $n=22$, the above codewords merge in a single codeword of weight $4$ 
\begin{align*}
\ldots10001|\textbf{1000000000010000000101}|001\ldots\\
\end{align*}
which, however it is not a minimum distance codeword, since $A(3)=4$. The \ac{PRC-LDPC} code instead assumes $d=4$ when $n=24$, for which $A(4)=10$. For the sake of brevity we only show the codeowords of weight $4$ deriving from the application of the results in Section \ref{sec:rules} to the codewords listed above
\begin{align*}
\ldots1|\textbf{000110000000000100000001}|01001\ldots\\
\ldots|\textbf{100011000000000010000000}|101001\ldots\\
\ldots100011|\textbf{000000000010000000101001}|\ldots\\
\ldots10001|\textbf{100000000001000000010100}|1\ldots\\
\end{align*}

This reasoning already shows that the weight distribution of \ac{PRC-LDPC} codes, at least for relatively small values of $n$ can be characterized starting from a very small portion of $\6m$ (i.e., 30 bits out of the total $2^{13}$). In this particular case, this portion of $\6m$ is that defined by Lemma \ref{lem:famiglia}. We show the initial values of $n(d)$ in Fig. \ref{fig:samples_vs_m}.



\begin{figure}
    \centering
    \resizebox{!}{8cm}{
\begin{tikzpicture}
  \begin{axis}[
%ytick={18,19,20,21,22,23,24,25,26,27,28,29},        
%yticklabels={,$19$,$20$,$21$,$22$,$23$,$24$,$25$,$26$,$27$,$28$,$29$},        %ytick={1,0.1,0.01,0.001,0.0001,0.00001,0.000001,0.0000001},
ymin = 18,
ymax= 35,
grid = both,
xmin=1,
xmax=8,
%xmode = log,
%ymode = log,
legend style={at={(1.02,1)},anchor=north west},
mark size=2pt,
xlabel={$\textcolor{white}{R'}d\textcolor{white}{R'}$},
ylabel={$n(d)$},
xticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
}]


\addplot[black, mark = x, line width=0.7pt]coordinates{
(2, 19)
(3, 19)
(3,21)
(4,21)
(4,24)
(5,24)
(5,29)
(6,29)
(6,31)
(7,31)
(7,34)
};%\addlegendentry{$q=2^{256}$};

 
%%%%%%%%%%%%%%%%%%

\end{axis}
\end{tikzpicture}}
    \caption{Minimum distance profile of the \ac{PRC-LDPC} code described by $\6e=[0,1,5,11,13]$.}
    \label{fig:samples_vs_m}
\end{figure}


The next family of \ac{PRC-LDPC} codes we consider is that described by $h(x)=1+x+x^3+x^{12}+x^{16}$. The separation vector is
\[
\6s=[1,2,9,4],
\]
and we notice that $s_{\max}=9$ exceeds the sum of all the other separations. This means that the hypotheses of Theorem \ref{the:zerozones} are not verified.

The portion of $\6m$ containing $\6h^*$ is
\[
\ldots,|111|0000000|\mathbf{10001000000001011}|000000000|1000001,\ldots
\]
and from Corollary \ref{cor:corsidon} we have that $n(6)\geq 34$. To be noticed that, since Remark \ref{rem:rul_int} was not respected, the comb-like structure as in Fig. \ref{fig:zonapettini} is not present on the right-hand side, even though it appears on the left-hand side.

